Tangent Images for Mitigating Spherical Distortion

In this work, we propose "tangent images," a spherical image representation that facilitates transferable and scalable $360^\circ$ computer vision. Inspired by techniques in cartography and computer graphics, we render a spherical image to a set of distortion-mitigated, locally-planar image grids tangent to a subdivided icosahedron. By varying the resolution of these grids independently of the subdivision level, we can effectively represent high resolution spherical images while still benefiting from the low-distortion icosahedral spherical approximation. We show that training standard convolutional neural networks on tangent images compares favorably to the many specialized spherical convolutional kernels that have been developed, while also scaling efficiently to handle significantly higher spherical resolutions. Furthermore, because our approach does not require specialized kernels, we show that we can transfer networks trained on perspective images to spherical data without fine-tuning and with limited performance drop-off. Finally, we demonstrate that tangent images can be used to improve the quality of sparse feature detection on spherical images, illustrating its usefulness for traditional computer vision tasks like structure-from-motion and SLAM.

==> main-paper/figures/semseg-results.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=1.0\linewidth, trim={0mm 0mm 0mm 0mm}, clip]{main-paper/images/semantic_segmentation_results.pdf}
\caption{\small Plot of our semantic segmentation results compared to prior work using RGB-D inputs from Stanford2D3DS.}
\label{fig:semseggraph}
\end{figure}
